A Token-level Text Image Foundation Model for Document Understanding

In recent years, general visual foundation models (VFMs) have witnessed increasing adoption, particularly as image encoders for popular multi-modal large language models (MLLMs). However, without semantically fine-grained supervision, these models still encounter fundamental prediction errors in the context of downstream text-image-related tasks, i.e., perception, understanding and reasoning with images containing small and dense texts. To bridge this gap, we develop TokenOCR, the first token-level visual foundation model specifically tailored for text-image-related tasks, designed to support a variety of traditional downstream applications. To facilitate the pretraining of TokenOCR, we also devise a high-quality data production pipeline that constructs the first token-level image text dataset, TokenIT, comprising 20 million images and 1.8 billion token-mask pairs. Furthermore, leveraging this foundation with exceptional image-as-text capability, we seamlessly replace previous VFMs with TokenOCR to construct a document-level MLLM, TokenVL, for VQA-based document understanding tasks. Finally, extensive experiments demonstrate the effectiveness of TokenOCR and TokenVL. Code, datasets, and weights will be available at https://github.com/Token-family/TokenFD.

==> Table/OCRBench.tex <==
\begin{tabular}{c|ccccccccccc}
        \toprule
        8B-Model & MM1.5 &POINT1.5 &GPT-4o &Gemini-1.5-Pro & GLM-4v  &Claude3.5 & InternVL2.5 \\
        \midrule
        Score & 635 &720 &736 & 754 & 776 &788 & 822 \\
        \bottomrule
    \end{tabular}
% \vspace{-1cm} % 添加垂直间距
\qquad
\begin{tabular}{c|ccccccccccc}
            \toprule
        8B-Model & TextMonkey & DocOwl-1.5 & TextHawk2 & TokenVL(ours) & MiniMonkey\\
        \midrule
        Score & 561 & 599 & 784 & \textbf{851} & 802\\
        \bottomrule
\end{tabular}


==> Table/ZS_VQA.tex <==
\begin{tabular}{l|c|ccc|ccc}
\toprule
\multirow{2}{*}{ Method } & \multirow{2}{*}{ \#Param } & \multicolumn{3}{c|}{ Document Analysis } & \multicolumn{3}{c}{ Image Understanding } \\
& & DocQA & ChartQA & InfoVQA & VQAv2 & GQA & OKVQA \\
\midrule
CLIP-L~\cite{CLIP} & 304 M & 22.3 & 23.6 & 25.0 & 72.8 & 61.2 & 55.8 \\
DINOv2~\cite{dinov2} & 632 M & 14.7 & 15.9 & - & - & 63.9 & - \\
SAM-L~\cite{SAM} & 632M & 13.9 & 15.0 & - & - & 51.0 & - \\
Vary~\cite{vary} & 525 M & 42.8 & 41.8 & - & - & 42.6 & - \\
RADIO-H~\cite{ranzinger2024radio} & 632M & 18.2 & 20.2 & 24.5 & 72.9 & 61.8 & 55.9 \\
UNIT~\cite{zhu2024unit} & 632M & 43.0 & 46.0 & 28.7 & 72.3 & 60.4 & 55.5 \\
\midrule
InternViT2.5~\cite{internvl} &300M&&&&\\
Ours & & & & & & &\\
\bottomrule
\end{tabular}
